Complementary Search of Fermionic Absorption Operators at Hadron Collider and Direct Detection Experiments

Instead of the energy recoil signal at direct detection experiments, dark fermion appears as missing energy at hadron colliders. For a fermionc dark sector particle that coupled with quarks and neutrino via absorption operators, its production at collider is accompanied by an invisible neutrino. We study in details the mono-$X$ (photon, jet, and $Z$) productions at the Large Hadron Collider (LHC). We start from the quark-level absorption operators to make easy comparison between the collider and direct detection experiments. In other words, we study the model-independent constraints on a dark fermion with absorption operator. In addition, the interplay and comparison with the possible detection at the neutrino experiments, especially Borexino, is also briefly discussed. We find that light nuclear target can provide the stronger constraints on both spin-dependent and spin-independent absorption operators.

==> mSymbol.tex <==
% mSymbol.tex : Personal Abbreviations on Mathematical Symbol
% Kai Ma (Shaanxi University of Technology)
% Email: makai@snut.edu.cn
%
% Created on Sat Nov 27 22:34:27 CST 2021
%
% Modified on 






% New commands  for reference  % 
\renewcommand{\eqref}[1]{Eq.~(\textcolor{red}{\ref{#1}}) }
\newcommand{\figref}[1]{Eq.~(\textcolor{brown}{\ref{#1}}) }
\newcommand{\tabref}[1]{Eq.~(\textcolor{purple}{\ref{#1}}) }




% Abbreviations for Text  %         
%
\def\ie{{\it i.e.}}
\def\etal{{\it et al.}}
\def\etc{{\it etc.\ }}
\newcommand{\kainote}[1]{\textcolor{red}{#1}}


%%%%%%%%%%%%%%%%%%%
% Abbreviations for Eviroment         %
%%%%%%%%%%%%%%%%%%%
\newcommand{\bew}{\begin{widetext}}
\newcommand{\enw}{\end{widetext}}
\newcommand{\bee}{\begin{equation}}
\newcommand{\ene}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\ena}{\end{eqnarray}}
\newcommand{\bes}{\begin{subequations}}
\newcommand{\ens}{\end{subequations}}
\newcommand{\ds}[1]{#1\!\!\!\slash}


\def\nn{\nonumber}
\def\nin{\noindent}




%%%%%%%%%%%%%%%%%%%
% Setting Abbreviations for Mathmatical Symbles           %
%%%%%%%%%%%%%%%%%%%

\def\Cslash{C\!\!\!\!\slash }
\def\Dslash{D\!\!\!\!\slash }
\def\Qslash{Q\!\!\!\!\slash }
\def\Hslash{H\!\!\!\!\slash }
\def\paslash{\partial\!\!\!\slash }
\def\pslash{p\!\!\!\slash }
\def\Aslash{A\!\!\!\slash }
\def\Bslash{B\!\!\!\slash }
\def\sslash{s\!\!\!\slash }
\def\Sslash{S\!\!\!\slash }
\def\to{\rightarrow}
\def\lr{\leftrightarrow}
\def\d{{\rm d}}


\def\cala{\mathcal{A}}
\def\calb{\mathcal{B}}
\def\calc{\mathcal{C}}
\def\cald{\mathcal{D}}
\def\cale{\mathcal{E}}
\def\calf{\mathcal{F}}
\def\calg{\mathcal{G}}
\def\calh{\mathcal{H}}
\def\cali{\mathcal{I}}
\def\calg{\mathcal{G}}
\def\calk{\mathcal{K}}
\def\call{\mathcal{L}}
\def\calm{\mathcal{M}}
\def\caln{\mathcal{N}}
\def\calo{\mathcal{O}}
\def\calp{\mathcal{P}}
\def\calq{\mathcal{Q}}
\def\calr{\mathcal{R}}
\def\cals{\mathcal{S}}
\def\calt{\mathcal{T}}
\def\calw{\mathcal{W}}
\def\calx{\mathcal{X}}
\def\caly{\mathcal{Y}}
\def\calz{\mathcal{Z}}

\def\scra{\mathscr{A}}
\def\scrb{\mathscr{B}}
\def\scrc{\mathscr{C}}
\def\scrd{\mathscr{D}}
\def\scre{\mathscr{E}}
\def\scrf{\mathscr{F}}
\def\scrg{\mathscr{G}}
\def\scrh{\mathscr{H}}
\def\scri{\mathscr{I}}
\def\scrj{\mathscr{J}}
\def\scrk{\mathscr{K}}
\def\scrl{\mathscr{L}}
\def\scrm{\mathscr{M}}
\def\scrn{\mathscr{N}}
\def\scro{\mathscr{O}}
\def\scrp{\mathscr{P}}
\def\scrq{\mathscr{Q}}
\def\scrr{\mathscr{R}}
\def\scrs{\mathscr{S}}
\def\scrt{\mathscr{T}}
\def\scru{\mathscr{U}}
\def\scrv{\mathscr{V}}
\def\scrw{\mathscr{W}}
\def\scrx{\mathscr{X}}
\def\scry{\mathscr{Y}}
\def\scrz{\mathscr{Z}}






% Abbreviations for Physical Unites %
\def\ev{\,{\rm eV}}
\def\kev{\,{\rm KeV}}
\def\mev{\,{\rm MeV}}
\def\gev{\,{\rm GeV}}
\def\tev{\,{\rm TeV}}
\def\pev{\,{\rm PeV}}
\def\aev{\,{\rm AeV}}

\def\nb{\,{\rm nb}}
\def\fb{\,{\rm fb}}
\def\pb{\,{\rm pb}}
\def\ab{\,{\rm ab}}

\def\inb{$\,{\rm nb}^{-1}$}
\def\ifb{$\,{\rm fb}^{-1}$}
\def\ipb{$\,{\rm pb}^{-1}$}
\def\iab{$\,{\rm ab}^{-1}$}








%\renewcommand{\title}[1]{\boldmath #1}

